COARSE3D: Class-Prototypes for Contrastive Learning in Weakly-Supervised 3D Point Cloud Segmentation

Annotation of large-scale 3D data is notoriously cumbersome and costly. As an alternative, weakly-supervised learning alleviates such a need by reducing the annotation by several order of magnitudes. We propose COARSE3D, a novel architecture-agnostic contrastive learning strategy for 3D segmentation. Since contrastive learning requires rich and diverse examples as keys and anchors, we leverage a prototype memory bank capturing class-wise global dataset information efficiently into a small number of prototypes acting as keys. An entropy-driven sampling technique then allows us to select good pixels from predictions as anchors. Experiments on three projection-based backbones show we outperform baselines on three challenging real-world outdoor datasets, working with as low as 0.001% annotations.

==> BMVC 22 - COARSE3D - arxiv/defines.tex <==
\newcommand{\todo}[1]{{\textcolor{red}{#1}}}
\newcommand{\QCc}[1]{\textcolor{blue}{[\textbf{Quan}: #1]}}
\newcommand{\RCc}[1]{\textcolor{purple}{[\textbf{RC}: #1]}}
\newcommand{\RLc}[1]{\textcolor{bicyclist}{[\textbf{Rong}: #1]}}

\newcommand{\QC}[1]{{\textcolor{blue}{#1}}}
\newcommand{\RC}[1]{\textcolor{purple}{#1}}
\newcommand{\RL}[1]{\textcolor{bicyclist}{#1}}

\newcommand{\add}[1]{\textcolor{orange}{#1}}
\newcommand{\edit}[2]{\textcolor{orange}{#2}}

\newcommand{\ourmethod}[1]{\textcolor{red}{OurFancyMethod}}


\definecolor{car}{rgb}{0.39215686, 0.58823529, 0.96078431}
\definecolor{bicycle}{rgb}{0.39215686, 0.90196078, 0.96078431}
\definecolor{motorcycle}{rgb}{0.11764706, 0.23529412, 0.58823529}
\definecolor{truck}{rgb}{0.31372549, 0.11764706, 0.70588235}
\definecolor{other-vehicle}{rgb}{0.39215686, 0.31372549, 0.98039216}
\definecolor{person}{rgb}{1.        , 0.11764706, 0.11764706}
\definecolor{bicyclist}{rgb}{1.        , 0.15686275, 0.78431373}
\definecolor{motorcyclist}{rgb}{0.58823529, 0.11764706, 0.35294118}
\definecolor{road}{rgb}{1.        , 0.        , 1.        }
\definecolor{parking}{rgb}{1.        , 0.58823529, 1.        }
\definecolor{sidewalk}{rgb}{0.29411765, 0.        , 0.29411765}
\definecolor{other-ground}{rgb}{0.68627451, 0.        , 0.29411765}
\definecolor{building}{rgb}{1.        , 0.78431373, 0.        }
\definecolor{fence}{rgb}{1.        , 0.47058824, 0.19607843}
\definecolor{vegetation}{rgb}{0.        , 0.68627451, 0.        }
\definecolor{trunk}{rgb}{0.52941176, 0.23529412, 0.        }
\definecolor{terrain}{rgb}{0.58823529, 0.94117647, 0.31372549}
\definecolor{pole}{rgb}{1.        , 0.94117647, 0.58823529}
\definecolor{traffic-sign}{rgb}{1.        , 0.        , 0.    }   


\definecolor{nus00}{rgb}{0.9607843137254902, 0.9411764705882353, 1.0}
\definecolor{nus01}{rgb}{0.5647058823529412, 0.5019607843137255, 0.4392156862745098}
\definecolor{nus02}{rgb}{0.23529411764705882, 0.0784313725490196, 0.8627450980392157}
\definecolor{nus03}{rgb}{0.0, 0.27058823529411763, 1.0}
\definecolor{nus04}{rgb}{0.0, 0.6196078431372549, 1.0}
\definecolor{nus05}{rgb}{0.27450980392156865, 0.5882352941176471, 0.9137254901960784}
\definecolor{nus06}{rgb}{0.38823529411764707, 0.23921568627450981, 1.0}
\definecolor{nus07}{rgb}{0.5019607843137255, 0.0, 0.0}
\definecolor{nus08}{rgb}{0.30980392156862746, 0.30980392156862746, 0.1843137254901961}
\definecolor{nus09}{rgb}{0.0, 0.5490196078431373, 1.0}
\definecolor{nus10}{rgb}{0.2784313725490196, 0.38823529411764707, 1.0}
\definecolor{nus11}{rgb}{0.7490196078431373, 0.8117647058823529, 0.0}
\definecolor{nus12}{rgb}{0.29411764705882354, 0.0, 0.6862745098039216}
\definecolor{nus13}{rgb}{0.29411764705882354, 0.0, 0.29411764705882354}
\definecolor{nus14}{rgb}{0.23529411764705882, 0.7058823529411765, 0.4392156862745098}
\definecolor{nus15}{rgb}{0.5294117647058824, 0.7215686274509804, 0.8705882352941177}
\definecolor{nus16}{rgb}{0.0, 0.6862745098039216, 0.0}



\definecolor{poss01}{rgb}{ 0.11764705882352941, 0.11764705882352941, 1.0 }
\definecolor{poss02}{rgb}{ 0.7843137254901961, 0.1568627450980392, 1.0 }
\definecolor{poss03}{rgb}{ 0.9607843137254902, 0.5882352941176471, 0.39215686274509803 }
\definecolor{poss04}{rgb}{ 0.0, 0.23529411764705882, 0.5294117647058824 }
\definecolor{poss05}{rgb}{ 0.0, 0.6862745098039216, 0.0 }
\definecolor{poss06}{rgb}{ 0.0, 0.0, 1.0 }
\definecolor{poss07}{rgb}{ 0.5882352941176471, 0.9411764705882353, 1.0 }
\definecolor{poss08}{rgb}{ 0.0, 1.0, 0.49019607843137253 }
\definecolor{poss09}{rgb}{ 0.0, 0.7843137254901961, 1.0 }
\definecolor{poss10}{rgb}{ 1.0, 1.0, 0.19607843137254902 }
\definecolor{poss11}{rgb}{ 0.19607843137254902, 0.47058823529411764, 1.0 }
\definecolor{poss12}{rgb}{ 0.9607843137254902, 0.9019607843137255, 0.39215686274509803 }
\definecolor{poss13}{rgb}{ 0.5019607843137255, 0.5019607843137255, 0.5019607843137255 }



\makeatletter
\newcommand{\car@semkitfreq}{4.08}
\newcommand{\bicycle@semkitfreq}{0.02}
\newcommand{\motorcycle@semkitfreq}{0.04}
\newcommand{\truck@semkitfreq}{0.21}
\newcommand{\othervehicle@semkitfreq}{0.16}
\newcommand{\person@semkitfreq}{0.18}
\newcommand{\bicyclist@semkitfreq}{1.11e-6}
\newcommand{\motorcyclist@semkitfreq}{5.53e-9}
\newcommand{\road@semkitfreq}{19.87}  %
\newcommand{\parking@semkitfreq}{1.47}
\newcommand{\sidewalk@semkitfreq}{14.39}  %
\newcommand{\otherground@semkitfreq}{0.39}
\newcommand{\building@semkitfreq}{13.26}  %
\newcommand{\fence@semkitfreq}{7.23}
\newcommand{\vegetation@semkitfreq}{26.68}  %
\newcommand{\trunk@semkitfreq}{0.60}
\newcommand{\terrain@semkitfreq}{7.81} %
\newcommand{\pole@semkitfreq}{0.28}
\newcommand{\trafficsign@semkitfreq}{0.06}
\newcommand{\semkitfreq}[1]{{\csname #1@semkitfreq\endcsname}}




